Binomial Tails for Community Analysis

An important task of community discovery in networks is assessing significance of the results and robust ranking of the generated candidate groups. Often in practice, numerous candidate communities are discovered, and focusing the analyst's time on the most salient and promising findings is crucial. We develop simple efficient group scoring functions derived from tail probabilities using binomial models. Experiments on synthetic and numerous real-world data provides evidence that binomial scoring leads to a more robust ranking than other inexpensive scoring functions, such as conductance. Furthermore, we obtain confidence values ($p$-values) that can be used for filtering and labeling the discovered groups. Our analyses shed light on various properties of the approach. The binomial tail is simple and versatile, and we describe two other applications for community analysis: degree of community membership (which in turn yields group-scoring functions), and the discovery of significant edges in the community-induced graph.

==> formulation.backup.tex <==
\section{Formulation}
\label{sec:form}

%This means in particular that, given a node that has d edges (has
%degree d), the other end of each edge is selected uniformly at random
%with replacement (repeated edges are possible).

%We use a similar model for a group.
%The event of interest is:

%For much of this work, the graph is
% unweighted.

An undirected unweighted graph $\G$ consists of a node set
$\nodeset$ and edge set $\edgeset$.  A group $\g$ is a subset of nodes
($\g \subseteq \nodeset$).  An edge (unordered pair of nodes) $\{u,v\}
\in \edgeset$ is referred to as an (incident) edge of the group $\g$
if $u \in \g$ or $v \in \g$.  We refer to the number of edges of a
group as the {\em degree} of the group (akin to degree of a node),
denoted by $\deg(\g)$. Thus, $\deg(\g) = |\{\{u,v\}\in \edgeset, \mbox{s.t. } \  u \in \g \ \mbox{or}  \ v
\in \g \}|$. To declutter notation, we often drop the generic group
$\g$ and simply write $\deg$, as we often do for other functions of
groups to be introduced.  If both ends of an edge are in the group
$\g$, we will call it an {\em internal} edge, and otherwise (exactly
one-end in $\g$) it's an {\em outgoing} edge. We refer to the number
of internal edges as the {\em internal degree}, and denote it with
$\din, \din \le \deg$.  Intuitively, a group that is dense inside and
sparse outside, \ie the observed ratio $\frac{\din}{\deg}$ is
relatively large, may correspond to a real-world community.

% meaning $\din$ is relative
%We are given a group of nodes as a candidate community (by an
%algorithm, or some process).

%Assume a given group $s$ has $\deg$ incident edges, \ie
%has {\em degree} $\deg$, and we observe in particular that $\din$ of
%such edges, $\din \le \deg$ 'fall inside' the group, i.e. both ends
%are inside the group.

%where the
%other end is also in group,

Now, given is a group (generated by some algorithm or process) with
degree $\deg$ and internal degree $\din$, and we are interested in the
probability of observing such an event by chance, which we formalize
next. We assume a uniform random model of connection as the {\em null}
(reference) model: for each of $\deg$ edges, one end is already in the
group, and the other end is picked from all vertices at random. Each
such pick is a random trial, so there are $\deg$ trials.  We define
the event of interest as: observing $\din$ or more internal edges, or
$\din$ of the trials pick a node in the group, out of $\deg$ trials.
If the probability of such event, according to the null model, is
tiny, or in other words it appears to be an extreme event, then we have
good evidence that the given group is special, in terms of density
inside relative to all group edges or outgoing edges (an indication of
community property), \ie this is unlikely to have happened by chance.
Note that, as is common when assessing statistical significance, we
are being conservative, and for example not asking for the probability
of the event of observing exactly (or around) $\din$ internal edges as
such point-events are often unlikely to begin with (there are many
possible values for $\din$).

% , and this is common
% statistical practice as well.

% and compute the probability of the tail
%event that we observed $\din$ {\it or more} internal edges, when the
%other end of each edge is picked uniformly at random (with
%replacement).

%\footnote{As is common practice for statistical tests, we use
%  the conservative one-sided event (that we observed no less than
%  $\din$ successes): the point-event of observing exactly $\din$
%  successes, may unsurprisingly obtain a low probability simply
%  because there are so many possible values for number of successes.
%}

%Let $\D$ denote the random variable for the number of
%internal edges under this null model (note: $0\le \D \le \deg]$).

%(based on number of nodes), the expected
% group-internal connection probability,

Let $\pn$ be the (expected) probability that the other end of a group
edge is in the group (a 'success'), which according to the null model
is $\pn=\frac{\gsize}{\nodes}$ ('expected' according to the null
model). We call this model the {\em node-based} model (an edge-based
model is described in Section \ref{sec:edgeway}).\footnote{If we don't
  allow self-edges, we could use the more precise $\pn=\frac{|\g| -
    1}{|\nodeset| - 1}$.} We refer to $\frac{\din}{\deg}$ as the {\em
  observed proportion}.  The tail probability,
$\mathtt{BinomialTail}(\deg, \din, \pn)$, that we observe $\din$ or
more successes out of $\deg$ independent attempts, with success
probability $\p=\pn$, is given by:

% remove event E  or another part to shorten it..
%  P(\E) = P(\D \ge \din| \mathtt{group \  with \ degree\ } \deg) =
  
\begin{equation}
\label{eq:binomial}    
  \mathtt{BinomialTail}(\deg, \din, \p) =  \sum_{i \ge d_{in}}
         {\deg \choose i} \p^i(1-\p)^{\deg-i}, \mbox{\ \ where, for the node-based model, }
         \p=\pn=\frac{|\g|}{|\nodeset|}
\end{equation}

The tail probability in a principled manner combines the connectivity
attributes of the group (degree and internal edges) and other context
(group and graph size). Note that for weighted edges, if they are
integers or roundable to integers, the graph can be treated as a
multigraph, and the statistics such as degree appropriately computed
by computing the multiple edges (a similar approach for computing
modularity).



%Let the random variable $\D$ denote the number of internal edges, and we
%seek the probability of the event $\D \ge \din$ given that the group
%has degree $\deg$, according to the following (random uniform) null
%model: the other side of each of the $\deg$ edges is picked uniformly
%at random (with replacement) (note: $0\le \D \le \deg]$).

%Intuitively, the lower this probability is, or the higher the
%surprise, the more confident we are that the group has meaningful
%(non-accidental) community structure (relatively dense internal and
%relatively sparse connections to outside, all relative to the null
%uniformly at random model).

% This tail probability has a simple formula.

\subsection{Evidence and Group Size}

Our original motivation was a principled method for scoring with a
preference for larger groups. Informally, larger groups should provide
more evidence of community structure assuming other properties such as
internal density remains roughly equal, since degree $\deg$ tends to
go up with larger groups.  However, the expected proportion $\p$
($\pn$) also goes up for larger groups, which can counteract $\deg$,
\ie the larger group could get a smaller significance.

For two isolated groups (no outgoing edges, or $\din=\deg$), where
nodes have similar (internal) degree in both groups, it is easy to
show that both situations can occur, as the following establishes. But
as long as the larger group is not too big, as a fraction of the
graph, indeed we obtain higher significance for the larger group:
\begin{prop}
  \label{prop:evidence}
For two groups with no outgoing edges, $\g_1$ and $\g_2$, $|\g_2| =
2|g_1|$, $\deg(\g_i)=\din(\g_i)=|\g_i|$ (node degree of roughly 1), the larger
group $\g_2$ obtains a lower tail probability (higher significance) if
and only if $|\g_1| < 1/4|\nodeset|$.  More generally, with
$|\g_2|=k|\g_1|, k > 1$, and $\deg(\g_i)=a|\g_i|, a > 0$, $\g_2$
obtains a higher significance iff $\frac{|g_1|}{|\nodeset|} <
k^\frac{-k}{k-1}$ (independent of $a$).
\end{prop}

For the proof, first for $k=2$, let $n=|\nodeset|$ and $|\g_1| = pn$,
thus $|\g_2| = 2pn,$ and $\deg(\g_1)=\din(\g_1)=|\g_1|=pn$, and
$\deg(\g_2)=\din(\g_2)=2pn$, and, from equation \ref{eq:binomial}, we
want to see when $p^{pn} > (2p)^{2pn}$, or $pn\log(p) > 2pn\log(2p)
\Rightarrow \log(p) > 2\log(2p)$, or $-\log(p) > 2\log(2) \Rightarrow
p < 1/4$. For general $k > 1$, replace $2$ with $k$ and insert $a$:
$p^{apn} > (kp)^{akpn} \Rightarrow \log(p) > k\log(kp) \Rightarrow \cdots$.

Similar patterns and proof applies to dense (isolated) groups such as
(near) cliques, \eg replace number of group edges with $0.5(pn)^2$,
and in this case the condition on the size of the larger group to
obtain higher significance becomes less strict (plausible, as $\din$
goes up quadratically).  Appendix \ref{app:resolution}, shows another
example, to illustrate a resolution-limit problem for the binomial
tail, where a larger group is deemed more significant although it may
be almost half as dense as a ratio (but with more internal edges). In
practice, it's also the case that all or most groups discovered are a
small fraction of the graph in number of nodes, and we empirically
find that the tail is typically well correlated with graph size in the
experiments of Section \ref{sec:exps}.

% As outoging edges are added, to the larger
% group for example, this preference over the larger group holds for
% some time.

\co{
We note that for two groups $\g_1$ and $\g_2$ with the same expected
and observed proportions (\ie $\p_1=\p_2, \q_1=\q_2$), the one with more
edges (group degree), also gets a higher significance for most ranges
of $d$. For example, both group may have 10 nodes, in a 100 node
graph, thus $\p_i=0.1$, and $\g_1$ can have $10$ inside and $10$
outgoing ($\q_1=0.5$), while $\g_2$ has 20 internal edges and 20
outgoing ($\q_2=0.5$ as well). This is seen from the upper and lower
bound expressions of \ref{eq:kl}, presented next.
}

\subsection{Approximation}

Equation \ref{eq:binomial} is simple to compute, but it is inefficient
for many groups in large graphs ($O(k|\edgeset|$ for $k$ groups), and
can lead to numeric (floating point) problems.  Indeed in our
experiments when we use the exact formulation we see considerable slow
down, of two orders of magnitude, even on relatively small graphs of
100s of nodes (Appendix \ref{app:syns}).  Efficient computation also
aids other applications of the tail such as node membership (Appendix
\ref{app:apps}), and a potential use for repeated evaluation as an
objective for community mining. The approximate bounds below also shed
light on the properties of the tail such as on group ranking and growth,
as we will see.

There exists a normal approximation to the binomial tail
\cite{experimenters}, and one could use generic bounds such as
Chebychev \cite{MotwaniR95}, but these proved to be inadequate for our
use case (based on experiments). The normal approximation works best
for expected proportions $\p$ near $0.5$ and when the number of trials
is very large \cite{experimenters}. On real world datasets, we find
that the expected proportion $\p$ is often relatively small (\eg below
0.10) and the observed (connection) proportion $\q=\frac{\din}{\deg}$
is relatively large.  Fortunately, the following upper and lower bound
on the tail probability is sufficiently tight and serves us well
\cite{arratia89, ash90}:


% $P(o \ge d' | d incident edges)$

% Why not a 'point' estimate?

% The event of interest: we observe a group with k edges internal k'
% outside. What's the probability of such 'an event' according to our or
% some null model.


% Define the event, any refs?

% notation

% motivate the event

% the exact formulation

% the approximatation, motivation

%For the approximation to the tail bound, upper bound from Arratia and Gordon
%\cite{arratia89, ash90} (both lower and upper are in \cite{ash90}).

\begin{align}
\nonumber  & \frac{1}{ \sqrt{2\deg} } \U \le \mathtt{BinomialTail}(\deg, \din, \p) \le \U, \mbox{ where } \\
  \label{eq:kl}
& \U = \exp(-\deg \KL(\q || \p)), \mbox{ where } \q=\frac{\din}{\deg} \mbox { \ \ \  (U is the upper bound on the tail probability), }
\end{align}

% where, $\U = \exp(-\deg \KL(\frac{\din}{\deg}, \p))$, and

where $\KL()$ is the (asymmetric) relative entropy function (or
Kullback–Leibler divergence): $\KL(q|| p) = q\ln \frac{q}{p} +
(1-q)\ln\frac{1-q}{1-p}$, where $\ln()$ denotes the natural logarithm
function.  The ratio of the observed to expected proportion, $\i(\g)
=\frac{\q(\g)}{\p(\g)}$, is handy in the analyses below, and we will
refer to it as the {\em intensity} of the group (intensity of the
community property).

% Section \ref{sec:good} below analyses the quality of the bounds.

Thus we simply need the readily available number of graph nodes, size
of the group, and its degree and internal degree to compute the
approximation to the tail, in O(1) time.

\subsection{Binomial Scores}

% Should we call it score or score ???

For convenience of scoring and comparisons, as the probabilities can
get tiny for good groups, we will use the negative log base 10 of the
above upper and lower tail probabilities, akin to Richter scale for
measuring the power of earthquakes (see \ref{sec:range} below), and
take the average for scoring and ranking the groups:

%\begin{equation}
  \begin{align}
\label{eq:approx} & \lscore(\g) =  \deg\KL(\frac{\din}{\deg}|| \p)/\ln(10) \hspace*{1in} \mbox{lower score of group $\g$, using the upper bound on tail probability} \\
\nonumber & \uscore(\g) =  \lscore(\g) + 0.5 \log_{10} (2\deg(\g)) \hspace*{0.8in} \mbox{upper score of group $\g$, via the lower bound on tail probability}
\end{align}

%\label{eq:approx}
%& \bscore =  0.5(\uscore + \lscore) \hspace*{1in} \mbox{{\em approximate binomial score: mean oxf the two}}

In our implementation, when $\deg \le 50$ we use the exact formula of
equation \ref{eq:binomial}, and otherwise the approximations from above:
\begin{align}
\label{eq:bn}
  \bsn(\g) = \begin{cases}
  -\log_{10}( \mathtt{BinomialTail}(\deg(\g),\ \din(\g),\ \pn(\g))),  \mbox{ \ \ \  when $\deg(\g) < 50$ } \\
  0.5(\uscore(\g) + \lscore(\g)), \hspace*{0.5in}  \mbox{ otherwise, where $\p = \pn = \frac{|\g|}{|\nodeset|}$
    \ \ \ {\em node-based binomial score} } 
  \end{cases}
\end{align}
Furthermore, if the observed ratio $q$ is not higher than the
expected, \ie when $q=\frac{\din}{\deg}\le \p$, we return 0 score
(insignificant).


Note that the arithmetic mean of upper and lower score corresponds to
(the negative log of) the geometric mean of the bounds on
probabilities. Next we use the upper and lower bounds to analyze the
accuracy of the approximation.


% \frac{1}{ \sqrt{2\deg} } \U \le \mathtt{BinomialTailProb}(\din, \deg, \p) \le \U,


%Section \ref{sec:edge-based} gives a close
%alternative of the null model. The following sections touch on several
%aspects.

\subsection{Range and Growth of Binomial Scores}
\label{sec:range}
Looking at the upper and lower bounds of equation \ref{eq:approx}, we
note that the score can grow as fast as roughly group degree $\deg$,
and in the experiments we do observe these ranges for the higher
scoring groups. Moreover, we also observe a positive correlation with
group size as anticipated (larger groups tend to have higher
$\deg$). The score also goes up with KL divergence and in particular
increases in proportion with log of the intensity, as the following
proposition formalizes.

\begin{prop}
\label{prop:incr}
  With $\q > \p$, where $0 < \p < \q \le 1$, KL divergence increases
  with increasing intensity $\i=\q/\p$. Therefore the approximate
  binomial score (either the upper or lower or their mean) increases
  with either increasing $\deg$, when KL remains the same or also
  increases, or with increasing intensity $\i$, when $\deg$ remains
  the same.
\end{prop}

The first term of KL divergence is increasing in intensity $\i$, but the
2nd term ($(1-\q)ln\cdots$) is (slightly) decreasing.  To show that KL increases with e$\i$,
we will take the derivative and show the derivaitve is positive, under two cases,
that either $\p$ or $\q$ is constant.


For fixed $\q$, and replacing
$\p$ by $\q/\i$, $\frac{\partial \KL(\q||\p)}{\partial
  \i}=\frac{\partial q\ln(\i)}{\partial \i} + \frac{\partial (1-\q)\ln\frac{1-\q}{1-\q/\i} }{\partial \i} =
q\ln(\i)+(1-\q)(\ln\frac{1-\q}{1-\q/\i})(1-\q)(-1)(1-\q/\i)^{-2}(\q)\i^{-2}$,
and note that both summands are positive: $q\ln(\i) > 0$ ($\i > 1$)
and $-\ln\frac{1-\q}{1-\q/\i} > 0$, since $\frac{1-\q}{1-p} < 1$ (and
other product factors in the 2nd term are non-negative:
$\q(1-\q)^2(1-\q/\i)^{-2}\i^{-2} \ge 0$. Similarly with $\p$ fixed,
replacing $\q=\p\i$ (and we assume $\q < 1$ here, so $\i$ can be
increased), $\KL(\q||\p)=p\i\ln\i+(1-p\i)\ln\frac{1-p\i}{1-p}$, and
the derivative is: $\p\ln(\i) + \p\i\ln(\i) +
(-\p)\ln\frac{1-\p\i}{1-\p}+(1-\p\i)(\frac{-\p}{1-p})\ln\frac{1-\p\i}{1-\p}$,
and all summands are positive under the assumptions $\i>1$ and $\p <
\p\i = \q < 1$.


The scores 1, 2, 3, $\cdots$ correspond respectively to chance (tail)
probabilities of 0.1, 0.01, 0.001, $\cdots$ (as we use log base 10),
thus a score of 1 corresponds to a fairly weak confidence (0.1
p-value), and each successive increment implies 10 times more
significance (akin to the Richter scale), and scores around 2 and
higher indicate increasingly strong confidence. In practice, we
observe many generated groups with scores well above 3, and basically
the score growing proportional to group degree $\deg$ for many of the
discovered groups.

% A score in 2 to 3 indicates borderline statistical significance
% (corresponds to relatively weak p-values of $\approx 0.1$ and
% $0.05$).


\subsection{Goodness of the Approximation}
\label{sec:good}

Scoring and ranking need not be so precise as we only use approximate
models of reality to assess significance, and often community
discovery tasks have an inherent subjective or imprecise component.
However, an approximation that is too far from the intended model
could defeat the initial motivation for using that approach.  Here we
will see that the approximation quality is promising, and furthermore
as the community property goes up (more precisely, when the
approximate lower and upper scores increase), the error in
approximation also improves.

A good way to assess the quality of the approximations above is to
look at the relative error, which can be achieved since we have both
an upper and a lower bound: Let $s(\g)$ be the actual binomial score
of group $\g$, and denote the relative error by $r(\g), r(\g) =
\frac{|s(\g) - \bsn(\g)|}{s(\g)}$ (for $s(\g) > 0$).  We can readily
see the following ($10\%$ or better) guarantee on the quality of the
approximation holds:

\begin{prop} Let $\tilde{r}(\g) = \frac{\uscore(\g) - \lscore(\g)}{\lscore(\g)} = \frac{0.5
    \ln(2\deg)}{\deg\KL(\q|| \p)}$. We have $r \le \tilde{r}$ and 1)
  $\tilde{r} < 0.1$ when $\KL() \ge 0.5$ and $\deg \ge 50$, and 2)
  (more generally), with $0 < \p < \q \le 1$, error $\tilde{r}()$ is
  reduced with increasing degree $\deg$ (with intensity fixed or
  increasing), or increasing intensity $\i$ (with degree fixed or
  increasing).
\end{prop}

The first claim, $r(\g)\le \tilde{r}(\g)$, follows from bounding the
numerator of $r(\g)$, \ie noting that $|s(\g) - \bsn(\g)| \le
\uscore(\g) - \lscore(\g)|$ (as both $s(\g)$ and $\bsn(\g)$ are in
$[\lscore(\g), \uscore(\g)]$), and for the denominator, $\lscore(\g)
\le s(\g)$. The second part follows from the expression for
$\tilde{r}$ and that KL increases with intensity from Proposition
\ref{prop:incr}.


\co{ When we look at a worst case version of relative error, \eg the
  ratio of the difference of the upper and lower score to the lower
  score, $\frac{\uscore - \lscore}{\lscore} = \frac{0.5
    \ln(2\deg)}{\deg\KL(\frac{\din}{\deg}|| \p)} $, we see that, as
  long as KL divergence is 0.5 or higher, the worst-case error,
  rapidly goes to 0 as degree grows, and, for example, for degree
  $\deg \ge 50$, the relative error is already below 10\%.  }


Note that we use the exact expression for the score when $\deg \le
50$, thus we framed the above claim for $\deg \ge 50$. The higher the
degree the lower the relative error, but we will focus briefly on the
KL divergence component of the error to see it is above say 0.5. The
divergence is above 0.5 (and easily exceeds 1) when the intensity $\i
\ge 2$, {\em and} $\p$ is relatively high, \ie $\p \ge 0.1$, \eg when
$\p = 0.1$, we need $\q \ge 0.21$, for a guaranteed below 10\%
relative error, when we ignore the additional help from $\deg$, and
error goes to below 5\% for $\deg\ge 100$. However, for a constant
intensity, the KL divergence goes down as $\p \rightarrow 0$.  For
instance, for $\p=0.01$ (a group of size hundredth of the graph), KL
divergence is above 0.5 only when $\q \ge 0.056$ (a requirement that
$\i \ge 5$).  In practice (on various datasets) many of the discovered
candidate communities do have high intensities, and one can argue that
more accurately scoring small groups with relatively low intensities
(low quality groups) is not as critical (see also Appendix
\ref{app:syns}).


For smaller groups, degree $\deg$ tends to also be small,\footnote{In
  particular, in (unweighted) sparse graphs (or
  $|\edgeset|=O(|\nodeset|)$), $\deg$ is a multiple of group size
  $\gsize$, assuming each node has roughly the average degree. } and,
looking at both the upper and lower bound on the score, we require a
higher intensity to attain a comparable score. This observation is
consistent with the intuition that the smaller the trials (the
evidence), the smaller the community quality score of a group should
be (see also Proposition \ref{prop:evidence}).


A tighter
(smaller) bound on relative error, as we use a midpoint, is:
$\max(\frac{\bsn(\g) -
  \lscore(\g)}{\lscore(\g)},\frac{\uscore(\g)-\bsn(\g)}{\bsn(\g)}))$,
but the above simpler expression gives an idea of the quality of the
approximation.  In practice, we could also use only the conservative
lower score, and also report the actual worst-case error $\tilde{r}()$
when we use the approximate binomial score. Our ranking experiments
showed little difference between using the lower or the average score,
as well as, in most cases, no difference in ranking quality when using the
exact \vs the approximate form of the score  (Appendix \ref{app:syns}) and
\ref{app:bin}).


%In the appendix, we report on the
%differences if any in the ranking when using lower (conservative) vs
%average of the upper and lower score.

% This is plausible since small $\p$ corresponds to fewer trials or
% smaller statistical evidence.

\subsection{A Null Model Based on Edge Proportion}
\label{sec:edgeway}

% Let $\m$ denote the number of edges in the graph.

In this null model, like above we are given a group with some number
of incident edges $\deg$, where we are free to pick the other end of
each such edge. Like above, we pick the other end of each such edge
independently with some probability $\p$, and $\p$ is different for
different groups. Here, the probability $\p$ is a function of the
number edges of the group $|\deg|$ and of the graph $|\edgeset|$ (\vs
the number of nodes of the group $|\g|$ and graph $|\nodeset|$), or
the relative 'chattiness' of the group, so a rough measure is
$\frac{\deg}{\m}$. More precisely, we use the following small variant,
which we denote by $\pe$:
\begin{equation}
\pe = \frac{\deg + \din}{2\m}
\end{equation}

To motivate the small difference in the definition of proportion,
imagine for each edge of the graph, we look at one end, randomly
picked, to see whether or not it's in group \g. Then the expected
number of nodes in $\g$ that we observe is $\frac{\deg + \din}{2}$
(out of $\m$ observations).  This is the same null model behind the
modularity objective \cite{newman_2004}, where the expected proportion
of internal edges, \ie both ends in $\g$, comes out to
$\pe^2$.\footnote{Symmetrically, one could define a modularity
  objective based on number of nodes, and a corresponding Louvain algorithm based on node
  proportion \vs edge proportion. See Appendix \ref{app:node_louvain}. }

We can replace $\pn$ with $\pe$ in Definition \ref{eq:bn} to get the
edge-based binomial score $\bse(\g)$, \ie the main difference is the
choice of the observed proportion $\p$. Note that $\frac{\deg +
  \din}{2}$ could also replace the number of trials $\deg$ in
Definition \ref{eq:bn}.

\subsection{A Comparison of the Two Models}
\label{sec:two_models}

What is the consequence of using one null model \vs the other?  The
implications are easier seen when we look at groups that have no
outgoing edges, \ie $\deg=\din$: the edge-based model may prefer
(internally) less dense groups (as $\pe$ can be smaller for
less dense group, irrespective of group size), compared to the
node-based model, which may prefer smaller (but possibly denser)
groups (as $\pn$ will be smaller or the exponent can be higher).
To illustrate this difference,
we present an extreme example in Figure
\ref{fig:comparare_null_models}(a).  For both groups, in either null
model, following equation \ref{eq:binomial}, the tail probability is
$\p^{\deg(\g)}$ (as $\din = \deg$). For the node-based model,
$\p_n(\g_1) = \p_n(\g_2) \implies \p^6_n(\g_1) < \p^3_n(\g_2)$ (where
$\pn(\g_1) = \frac{|\g_1|}{|\nodeset|} = \frac{4}{8} = \pn(\g_2)$).
For the edge-based model, $\p_e(\g_1)=\frac{2}{3} >
\p_e(\g_2)=\frac{1}{3}$, and $(\frac{2}{3})^6=(\frac{4}{9})^3 >
(\frac{1}{3})^3$. In this example, the node-based model prefers the
group that looks more like a community (both groups are isolated, but
group 1 is denser).

The node set $\nodeset$ grows in Figure
\ref{fig:comparare_null_models}(b), but no new edges are added, and
since $\p_n(\g_i)$ shrink ( have $\p_n(\g_1) = \p_n(\g_2)$), we see
that the significance of both groups under the node-based null model
(binomial score) grows, but score grows faster for group 1, while
there is no difference in the groups' scores in the edge-based
model.  Finally, in Figure \ref{fig:comparare_null_models}(c), as
outgoing edges are added to $\g_1$, the preference of $\g_1$ over
$g_2$ decreases, though $\g_1$ may still be preferred: this depends on
the 'value' of an internal edge \vs an outgoing edge, which in turn
depends on $|\nodeset|$ relative to $|\g_1|$ (or $\pn$). On the other
hand, in the edge-based model, the preference of $\g_2$ over $\g_1$
only grows. We can see that the edge-based model can have an advantage
here: it can prefer isolated groups with good density, while the
node-based model may prefer smaller dense groups that nevertheless
have many outgoing edges (less community-like to the naked eye).


%and we can verify that $\p^6_e(\g_1) > \p^5_e(\g_2)$ (\ie
%$\p^6_e(\g_1)=(\frac{6}{11})^6 > (\frac{5}{11})^5$).


\begin{figure}[!htbp]
\begin{center}
\leavevmode   % leave vertical mode?? 
%\epsfxsize=2.5 in
%\epsfysize=1.5 in
\subfloat[Graph with two groups ($\nodes=8$, $|\edgeset|=9$)]
         {\includegraphics[width=5cm,height=2.5cm]{dir_figs/two_groups.png}}
\subfloat[More nodes added to the graph]
         {\includegraphics[width=5cm,height=2.5cm]{dir_figs/two_groups_with_additional_nodes.png}}
\subfloat[Outgoing edges added to group 1]
         {\includegraphics[width=5cm,height=2.5cm]{dir_figs/two_groups_additional_edges.png}}
\end{center}
%\vspace{-.2in}
\caption{Example graphs where the node-based binomial model 'prefers'
  group $\g_1$ (\ie scores group 1 higher), but the edge-based model
  prefers group $\g_2$. In all three cases, $\pn(\g_1) = \pn(\g_2)$,
  and for graphs in (a) and (b), for both groups and in either node-
  or edge-based model, the tail probability is $\p^{\deg(\g)}$ (as
  $\din = \deg$).  See text for further explanations.}
\label{fig:comparare_null_models} % synthetic experiments
\end{figure}

We have observed on several datasets that, as might be expected, the
rankings by the two techniques are highly correlated (\eg Spearman
rank correlation of over 0.99 on 5000 groups from Amazon co-purchase
dataset in SNAP \cite{leskovec2016snap}).  In another experiment, on a
few graphs derived from network communications, we observed that if we
take the maximum of the two scores, and use 1.5 as a threshold on
score (corresponding to roughly 95\% confidence), we observed that we
get 5\% more groups deemed significant than if we use either measure
in isolation.

% i am pretty sure this is not true any more (for the global score, we take max):
% 
% In the experiments section we take the
% maximum of two scores as the Binomial score of a group.


\subsection{A Global Bound}
\label{sec:global}

The above null models were conditional on an observed group, \ie {\em given} a group with
certain size $k$ and degree degree $\deg$ (event $A$), we sought the
probability of observing $\din$ or more internal edges (event $B$).
The graph can be big and it may not be so surprising (so unlikely) to
observe such a group in a large graph. Here, we want to add more
context and account for graph size. The union bound (Boole's
inequality), \ie the probability of a disjunction is bounded by the
sum of component probabilities \cite{MotwaniR95}, gives us an upper bound on the
probability of the event $C$, that we observe {\em one or more groups
  (\ie subsets) of size $k$ with degree $\deg$ and internal degree $\din$ or more}:
\begin{align}
\nonumber P(C) & \le \sum_{\g \subseteq \nodeset, |\g|=k}  P(A) P(B|A), \mbox{\ from the union bound } \\
\nonumber P(C) & \le {|\nodeset| \choose k}  P(B|A) \mbox{\ \ \ \ \ \ (as $P(A) \le 1$) } \\
\label{eq:gb}  & = {|\nodeset| \choose k} \mathtt{BinomialTail}(\deg, \din, \p)
\end{align}
where $P(B|A)$ is given by equation \ref{eq:binomial}. We can define a
corresponding score, {\em global} binomial score, by taking the
negative log. We note that $\ln({|\nodeset| \choose k})$ can be
efficiently approximated using Sterling's formula for the factorial.

In our experiments, on synthetic datasets with relatively small groups
and graphs, the global binomial score goes to $\le 0$ (as the upper
bound of \ref{eq:gb} reaches and exceeds 1.0), while the binomial
effectively ranks the groups. On the real-world graphs data sets, we
did not observe a significant difference between the two (see Appendix
\ref{app:bin}).\footnote{To get a somewhat tighter bound, instead of
  replacing with 1.0, one could replace $P(A)$ with probability of the
  event of observing a size $k$ group with degree $\le \deg$. This
  requires a further generative assumption on the overall graph and
  does not purely reward community structure anymore, but how unlikely
  a group size and degree is with respect to the choice of graph
  generation. We didn't observe a difference when we used the uniform
  Erdos-Reny model for graph generation estimating $P(A)$.  } Ixn
practice, one can use the more conservative bound of \ref{eq:gb} for
filtering and/or labeling and ranking candidate groups, with a
possible fall-back to plain binomial score for ranking the borderline
cases.


\subsection{Other Scoring Methods and a Discussion}
\label{sec:methods}

We compare ranking via the binomial score $\bsn(\g)$ with several simple
scoring methods:
\begin{enumerate}
\item Modularity (group-wise) \cite{newman_2004,leskovec2010}: $\qi(\g) = \frac{\din(\g)}{\m} - p_e(\g)^2$, is the
  fraction of observed internal edges minus a expectation for such
  fraction, according to the null model of Section \ref{sec:edgeway}.
\item Conductance \cite{malik2000}: $\frac{ \deg(\g) - \din(\g) }{ \deg(\g) + \din(\g) }$ (the lower the better).\footnote{In the denominator, the minimum of degree and internal degree for $\g$ and its complement
  (rest of the graph, $\nodeset - \g$) is used.
  Since $\g$ is substantially smaller than half of graph in our experiments,
  we do not see a difference in conductance value.  }
\item Triangle participation ratio (TPR) \cite{leskovec2012icdm}: for a group $\g$:  $TPR(\g) =
  \frac{|\{u: \exists t \in triangles(\grp), \ u \in t \}|}{|\grp|}$,  where \\
  $triangles(\grp)= \{\{u, v, w\}:\{u, v, w\} \subseteq \grp, \{\{u,v\}, \{v,w\}, \{w,u\}\} \subseteq \edgeset \}$
\item Descending group size (number of nodes in the group, Size)
\end{enumerate}

% the expected number of such edges in a random graph with identical
% degree sequence

%f(S) = cS / 2mS +cS  measures the fraction 2mS +cS
% of total edge volume that points outside the cluster [27].

%\cite{leskovec2012icdm}

We report correlation with group size per our motivation to bias
rankings towards larger groups. We also compare with ranking using
plain group size (largest first) as a baseline because in several
datasets and parameter settings this baseline (or its reverse) does
very well and sheds light on the nature of the specific ranking
problem.  We also report on the reverse (smallest first) in a few
cases.

We compare against $\qi()$ since we expect $\qi()$ to correlate with group
size as well, and it shares some similarity with the Binomial score:
it is also a function (the difference) of a candidate group's internal
edges \vs an expectation of such.  It can be readily available when we
use the Louvain algorithm and has been used in ranking comparisons
\cite{leskovec2012icdm,leskovecNature2018}. We note that the original
modularity formulation sums per-group differences over all groups to
assess an entire partitioning while we are using the group-wise
component of modularity for ranking groups.


Among a variety of simple scoring techniques tested, Yang and Leskovec
found that conductance and TPR performed among the best (one
reflecting internal density, another reflecting external separation)
\cite{leskovec2012icdm} and conductance in particular has been used
often as an objective for community discovery
\cite{seedSets06,fortunato2009}. Note that among these methods, only
TPR requires some nontrivial algorithm to compute.


\subsection{Discussion}
\label{sec:discuss}


Each technique has pluses but also shortcomings. TPR is an imperfect
measure of density inside the group and ignores outgoing edges. Note
also that TPR can be a perfect 1.0, and yet the internal density
($\din$) of a group can have much room for improvement. We see the
issue of tied scores often for TPR in the experiments. Both TPR and
conductance are 'normed' measures that factor out (ignore) group size
or number of connections (statistical evidence). Figure
\ref{fig:examples} show several groups with the same (perfect)
conductance of 0.0 and/or perfect TPR of 1.0 with varying sizes and
internal densities. We note that under stability and possibly
perturbation analysis tool, these structures may also obtain similar
scores since they may be rediscovered under multiple runs.  But
intuitively or at least in some tasks (like ours), one prefers larger
sizes and higher internal densities. We saw that the binomial score is
sensitive to increasing internal edges as well as overall degree.

% Tied scores, \eg TPR on
% several scenarios in our experiments, also present a drawback: they
% can lead to no ranking.

% ratio of observed connection probability to expected, $\frac{q}{\p}$,

The binomial score provides a principled way of combining internal and
outgoing edges and taking into account some of the other contextual
information (group and graph size). However, the approximations
inherent in using the tail, in equations of \ref{eq:approx}, or in the
union bound of equation \ref{eq:gb} may weaken the testing
(discriminative power and coverage). We observe these possibilities in
extreme cases in synthetic experiments (Appendix \ref{app:syns} and
\ref{app:bin}). It is also possible that real-world groups enjoy high
evidence, easily passing the significance threshold, and for those
passing the significance threshold (\eg a score above 2 or 3), the
binomial score may become a blunt instrument for ranking purposes.  We
conduct experiments on synthesized and real-world networks to shed
light on these possibilities and some of the issues will be explicitly
raised and discussed. Note that intensity score of $\i(\g) =
\frac{\q(\g)}{\p(\g)}$ (from Section \ref{sec:good}), is another
measure of strength of the (community) property. This score ignores
the raw degree counts (the support or the evidence), akin to
conductance and TPR. As an example, a group A may have a high
intensity of 10 ($\frac{q}{\p}=10$), but a binomial score of only 2,
while another group B may have an intensity of 2, but high binomial
score of 5: group B is larger than A, and has many internal edges
(providing much statistical evidence of community) but also external
edges, and subjectively, to the human eye, group A may seem more of a
community.  However, using intensity alone can become too biased
toward small or insignificant groups (this measure is called ratio
modularity in \cite{leskovec2010}).  In practice, likely multiple
measures are needed and should be presented to the user. For example,
one possibility is to filter by a confidence threshold, and rank what
remains by a measure of intensity.  We leave exploration of intensity
and combinations to future work. See also \cite{leskovecNature2018}
for combination techniques.


All these measures ignore how the internal connectivity is spread. For
instance, a given group might have a small internal cut, \ie may be
separable into two good nearly-sized groups via removing only a few
edges (a dumbbell shape, imbalanced group).  Or some single or few
nodes may have most of the internal connections of a group (\eg star
or core-priphery structure), while intuitively a more balanced spread
of the internal edges is preferred. The scoring techniques do rely on
the group generation technique to discover some good quality groups,
possibly mixed with poor quality ones, and the task is to highly rank
the best from among what is given, where what constitutes 'best' can be
application specific.  See also Appendix \ref{app:resolution} on
scoring groups based on aggregating the strength of membership-level
scores of individual nodes, which, as explained, may lead to more
balanced groups.

\co{
  
To discuss, some of the issues:
\begin{itemize}
  \item the problem with normalization: ignores size for our motivation
  \item Tied scores (several scoring techniques can exhibit this
    problem in different situations)
  \item Binomial score, range of valid values (power?),
    evidence/significance vs 'extremeness', could be too conservative
    (if we use lower bound), etc..? Also, it's for the overall group
    (some vertices may not really belong, or the could be small
    cuts), we are at mercy of the group generation technique here...
  \item Is there a problem to solve: maybe they all do well in
    practice?? Also, lack of groundtruth issues??
\end{itemize}
}


\begin{figure}[!htbp]
\begin{center}
\leavevmode   % leave vertical mode?? 
%\epsfxsize=2.5 in
%\epsfysize=1.5 in
\subfloat{\includegraphics[width=15cm,height=2.5cm]{dir_figs/examples.png}}
\end{center}
%\vspace{-.2in}
\caption{All groups are isolated (no outgoing edges) and have perfect
  conductance of 0. The first two on the left have 0 TPR (no
  triangles), and the remaining three groups have a perfect TPR of
  1.0.}
\label{fig:examples} % synthetic experiments
\end{figure}



% \subsection{Extension 2: Further Applications of Binomial Modeling}


\co{

In this null model, given a group, again one end of each incident edge
is fixed onto a node in the group, while the other is picked
independently at random.


However, in this  model,


Here, we can imagine $\m$ edges lined on top of one another
horizontally (in ladder format), and we observe on the left side that
$\deg$ left ends of edge (on the left side) happen to be in the
group. Then if the right side of each edge is also picked
independently at random according to roughly the same probability we
have binomial event.


according to similar
distribution

one end belongs to the group. Therefor the probability that an
end is picked from the group is $\p = \frac{\deg}{m}$.



and we ask
out of such edges, what’s the probability that we observe $\din$x or more
ends be in the group as well.  Pick or try up to d, as there are d
incident edges.



% where, $ U = exp(-\deg D(k/t, p))  $


% 1/(sqrt(2t)) U <= prob(k, t, p) <= U, where U=exp(-t D(k/t, p)), where
% D is relative entropy, and t is number of 'tries', and k are
% successes, so q=k/t is the 'precision'.

And we want to show the score, or the negative log of above, goes up
as function of group size, assuming say a sparse graph with degree d
avg. t in above is number of incident edges of the grp and p is
relative size of the group to total number of nodes n.

Lets rewrite as: prob(p*n*d, p*n*d, p), p is alpha or fraction of on n
nodes internal the group, p * n is group size.  lets assume all nodes
have degree d and that all incident edges fall both sides in the
group.

Lower score is L = t * D( k / t, p ) or p * n * d * D(1.0, p), and upper score is
is    L  + log( sqrt(2pnd) )   ( note: a >= 1/n )

( btw the diff ratio is:   [upper-score - lower-score] / upper-score, or

below n is num trials (or t above):

ratio = log(sqrt(2n)) / [ log(sqrt(2n)) + n + D(observed prob , expected prob ) ] 

since log sqrt(2n) is much smaller than n, we can see the fraction
diminishes quickly... and ratio <= log(sqrt(2n)) / [ log(sqrt(2n)) + n ] 

)



For the upper bound, the 2nd term increases as size of the group size
or p increases. For L,

D(k/t, p) = D(1, p) = 1.0 * log(1.0 / p) = -log(p), so L is
-ndplog(p), and -plog(p) peaks around p~0.4.

Now, assume q=k/t was high, but not 1.0, and p approaches it. Lets take
other values for q.. D(q, p)=qlog(q/p)+(1-q)log((1-q)/(1-p))

% }

% refs for bounds:

% https://en.wikipedia.org/wiki/Binomial_distribution
% https://en.wikipedia.org/wiki/Binomial_distribution#Tail_bounds

% # This tutorial:

% R. Arratia and L. Gordon: Tutorial on large deviations for the
% binomial distribution,
% Bulletin of Mathematical Biology 51(1) (1989), 125–131 [1].
% Robert B. Ash (1990). Information Theory. Dover Publications. p. 115

}

